Toward Low-Burden Image-Based Dietary Assessment Through Human-AI Collaborative Correction

Image-based dietary assessment can automate initial food logging, but meal photographs often leave food identity, hidden ingredients, preparation, and portion uncertain, making correction a recurring part of use. We introduce Human-AI Collaborative Correction, which reframes correction as communicate intent $\rightarrow$ regenerate $\rightarrow$ verify: users express what should change through text, voice, or guided clarification, the AI regenerates the linked dietary record, and users verify the result. In a within-participant study with 30 participants, compared with conventional Manual Search-and-Edit Correction, collaborative correction was associated with lower workload (Raw TLX: 35.83 vs. 55.00; p < .001), 21.0% lower recorded usage time, 51.1% fewer recorded clicks, and more favorable user-experience ratings; 90.0% preferred it overall. An exploratory nutrient analysis also found lower energy MAE. These findings support intent-driven regeneration as a promising interaction pattern for reducing correction burden while preserving user verification and making image-based dietary tracking easier to sustain.

==> figures/correction_architecture.tex <==
% Editable architecture schematic; original supplied PDF is retained separately.
\begingroup
\small
\setlength{\fboxsep}{7pt}
\fbox{\parbox{0.94\linewidth}{\centering
  \textbf{DietAI24 assessment engine}\par\smallskip
  Meal image + optional language context\quad$\rightarrow$\quad GPT-5.4 + FNDDS retrieval\par
  Current record: food codes/descriptions, portion codes/descriptions, gram weights, nutrients
}}
\par\smallskip
$\downarrow$\quad Current food and portion representations\quad$\downarrow$
\par\smallskip
\begin{minipage}[t]{0.48\linewidth}
  \centering
  \fbox{\parbox[t]{0.88\linewidth}{\raggedright
    \textbf{Quick Clarification}\par\smallskip
    Four GPT-5.4 audit agents:\par
    Ingredient Confirmation Agent\par
    Missing Ingredient Agent\par
    Added Fat, Sauce, or Seasoning Agent\par
    Portion Review Agent\par\smallskip
    Output: ranked candidates for user selection
  }}
\end{minipage}\hfill
\begin{minipage}[t]{0.48\linewidth}
  \centering
  \fbox{\parbox[t]{0.88\linewidth}{\raggedright
    \textbf{Visualized Portion Size}\par\smallskip
    FNDDS food and portion descriptions\par
    $\downarrow$\quad GPT-Image-2\par
    Visual references linked to portion options\par\smallskip
    Output: user-selected portion code and description
  }}
\end{minipage}
\par\medskip
\fbox{\parbox{0.94\linewidth}{\centering
  \textbf{Correction inputs}\par\smallskip
  Text/Voice Feedback + selected Quick Clarification candidates + selected visual portion options\par
  Selections stage context; explicit submission authorizes regeneration.
}}
\endgroup


==> figures/correction_concept.tex <==
% Editable conceptual diagram; original supplied PDF is retained separately.
\begingroup
\small
\setlength{\fboxsep}{8pt}
\noindent
\begin{minipage}[t]{0.48\linewidth}
  \centering
  \textbf{Manual Search-and-Edit Correction}\par\medskip
  \fbox{\parbox{0.88\linewidth}{\centering
    Provisional record + meal knowledge\par\smallskip
    $\downarrow$\par\smallskip
    Search the food database\par\smallskip
    $\downarrow$\par\smallskip
    Select food entries\par\smallskip
    $\downarrow$\par\smallskip
    Edit portions, weights, and components\par\smallskip
    $\downarrow$\par\smallskip
    Review and save the record
  }}\par\medskip
  Search, select, and edit fields
\end{minipage}\hfill
\begin{minipage}[t]{0.48\linewidth}
  \centering
  \textbf{Human--AI Collaborative Correction}\par\medskip
  \fbox{\parbox{0.88\linewidth}{\centering
    Provisional record + meal knowledge\par\smallskip
    $\downarrow$\par\smallskip
    Communicate correction intent\par\smallskip
    $\downarrow$\par\smallskip
    Explicitly submit correction context\par\smallskip
    $\downarrow$\par\smallskip
    AI regenerates linked record fields\par\smallskip
    $\downarrow$\par\smallskip
    Verify; accept or request another revision
  }}\par\medskip
  Communicate intent, regenerate, and verify
\end{minipage}
\par\medskip
{\footnotesize Schematic operations; box counts do not represent measured actions or effort.\par}
\endgroup


==> figures/correction_control_flow.tex <==
% Native LaTeX flow supplement; the supplied architecture PDF is preserved.
\begingroup
\setlength{\fboxsep}{4pt}
\footnotesize
\fbox{\parbox[c][0.42in][c]{0.16\linewidth}{\centering Assemble\\correction context}}
\hfill$\rightarrow$\hfill
\fbox{\parbox[c][0.42in][c]{0.13\linewidth}{\centering User explicitly\\submits}}
\hfill$\rightarrow$\hfill
\fbox{\parbox[c][0.42in][c]{0.13\linewidth}{\centering DietAI24\\regenerates}}
\hfill$\rightarrow$\hfill
\fbox{\parbox[c][0.42in][c]{0.13\linewidth}{\centering Revised\\record}}
\hfill$\rightarrow$\hfill
\fbox{\parbox[c][0.42in][c]{0.13\linewidth}{\centering User\\verifies}}
\par\smallskip
After verification: \textbf{accept} the record, or
\textbf{return to context assembly} for another revision.
\endgroup

